Fermi and Coulomb correlation effects upon the interacting quantum atoms energy partition

The Interacting Quantum Atoms (IQA) electronic energy partition is an important method in the field of quantum chemical topology which has given important insights of different systems and processes in physical chemistry. There have been several attempts to include Electron Correlation (EC) in the IQA approach, for example, through DFT and Hartree-Fock/Coupled-Cluster (HF/CC) transition densities. This work addresses the separation of EC in Fermi and Coulomb correlation and its effect upon the IQA analysis by taking into account spin-dependent one- and two-electron matrices $D^{\mathrm{HF/CC}}_{p\sigma q \sigma}$ and $d^{\mathrm{HF/CC}}_{p\sigma q\sigma r\tau s\tau}$ wherein $\sigma$ and $\tau$ represent either of the $\alpha$ and $\beta$ spin projections. We illustrate this approach by considering BeH$_2$,BH, CN$^-$, HF, LiF, NO$^+$, LiH, H$_2$O$\cdots$H$_2$O and C$_2$H$_2$, which comprise non-polar covalent, polar covalent, ionic and hydrogen bonded systems. The same and different spin contributions to ($i$) the net, interaction and exchange-correlation IQA energy components and ($ii$) delocalisation indices defined in the quantum theory of atoms in molecules are carefully examined and discussed. Overall, we expect that this kind of analysis will yield important insights about Fermi and Coulomb correlation in covalent bonding, intermolecular interactions and electron delocalisation in physical chemistry.

==> tablaVeeInter.tex <==
%\vspace{3cm}
\begin{sidewaystable}
\vspace*{12.0cm}
\caption{Interatomic electron-electron repulsion potential energy
($V_{ee}^{\mathrm{A}}$)
together with 
$V_{\mathrm{ee}}^{\mathrm{A} \sigma \sigma}$ and
$V_{\mathrm{ee}}^{\mathrm{A} \sigma \tau}$ ($\sigma \neq \tau$) 
for the molecules addressed in this work. The exchange-correlation
($V_{\mathrm{XC}}^{\mathrm{A} \sigma \sigma}$)
and its spin contributions are reported too. The data for the lighter
atom are displayed in the upper row of every system.
Atomic units are used throughout.}

%\vspace*{-1.0cm}

\begin{center}
\hspace*{-2.0cm} \begin{tabular}{l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l}
\hline
 & \multicolumn{8}{|c}{HF} & \multicolumn{12}{|c}{HF/CC} \\
\hline
System & \multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{AB}}$} & 
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{AB} \sigma \sigma}$} &
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{AB} \sigma \tau}$} & 
\multicolumn{2}{c|}{$V_{\mathrm{X}}^{\mathrm{AB} \sigma \sigma}$} & 
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{AB}}$} & 
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{AB} \sigma \sigma}$} &
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{AB} \sigma \tau}$} &
\multicolumn{2}{c|}{$V_{\mathrm{XC}}^{\mathrm{AB}}$} &
\multicolumn{2}{c|}{$V_{\mathrm{XC}}^{\mathrm{AB} \sigma \sigma}$} &
\multicolumn{2}{c}{$V_{\mathrm{XC}}^{\mathrm{AB} \sigma \tau}$} \\
\hline
\ce{BeH2} & 1&638273 & 0&781240 & 0&857033 & $-$0&075793 & 1&636422 & 0&780519 & 0&855902 & $-$0&079706 & $-$0&077546 & $-$0&002163 \\
%%%%%%%%%%%%%%%%%%%%%%%%%       %%%%%%%%%%%%%%%%%%%%%%%%%
\ce{BH} & 2&707343 & 1&275326 & 1&432016 & $-$0&156690 & 2&699614 & 1&271114 & 1&428500 & $-$0&163909 & $-$0&160647 & $-$0&003261 \\
%%%%%%%%%%%%%%%%%%%%%%%%%       %%%%%%%%%%%%%%%%%%%%%%%%%
\ce{CN-} & 17&055056 & 8&236270 & 8&818786 & -0&564832 & 17&158218 & 8&271384 & 8&886834 & -0&516372 & -0&565911 & 0&049539 \\
%%%%%%%%%%%%%%%%%%%%%%%%%       %%%%%%%%%%%%%%%%%%%%%%%%%
\ce{LiF} & 6&825120 & 3&390184 & 3&434938 & $-$0&044754 & 6&833302 & 3&393334 & 3&439968 & $-$0&046788 & $-$0&046710 & $-$0&000077 \\
%%%%%%%%%%%%%%%%%%%%%%%%%       %%%%%%%%%%%%%%%%%%%%%%%%%
\ce{HF} & 1&023441 & 0&440378 & 0&583064 & $-$0&142687  & 1&068421 & 0&459840 & 0&608582 & $-$0&146621 & $-$0&147681 & 0&001061 \\
%%%%%%%%%%%%%%%%%%%%%%%%%       %%%%%%%%%%%%%%%%%%%%%%%%%
\ce{NO+} & 21&067665 & 10&167070 & 10&900594 & $-$0&733525 & 21&234727 & 10&225648 & 11&009074 & $-$0&690796 & $-$0&737113 & 0&046313 \\
%%%%%%%%%%%%%%%%%%%%%%%%%       %%%%%%%%%%%%%%%%%%%%%%%%%
\ce{LiH} & 1&225795 & 0&593678 & 0&632118 & $-$0&038439 & 1&223486 & 0&592538 & 0&630948 & $-$0&040246 & $-$0&039328 & $-$0&000918 \\
%%%%%%%%%%%%%%%%%%%%%%%%%       %%%%%%%%%%%%%%%%%%%%%%%%%
\ce{HC#CH} & 0&000000 & 0&000000 &   0&000000 &   0&000000 &   0&000000 &   0&000000 &   0&000000 & $-$0&000000 & $-$0&000000 & 0&000000 \\
\ce{H2O\bond{...}H2O} & 0&000000 &   0&000000 &   0&000000 & 0&000000 &   0&000000 &   0&000000 & $-$0&000000 & $-$0&000000 & 0&000000 \\
\hline
%\hline
%\ce{CH3.} & 0&000000 &  0&000000 & 0&000000 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}  \\
%\ce{CH3CH2.}  & 0&000000 & 0&000000 & 0&000000 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}  \\
%\ce{(CH3)2CH.} & 0&000000 & 0&000000 & 0&000000 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}   \\
%\ce{(CH3)3C.}  & 0&000000 & 0&000000 & 0&000000 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---}  & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}  \\
\end{tabular}
\end{center}
\label{tab:VeeIntra}
\end{sidewaystable}%

\thispagestyle{empty}
\thispagestyle{empty}


==> tablaVeeTotal.tex <==
\thispagestyle{empty}
\thispagestyle{empty}
\begin{sidewaystable}
\caption{Total electron-electron potential energy ($V_{ee}^{\mathrm{total}}$)
along with its same and different-spin contributions 
$V_{\mathrm{ee}}^{\sigma \sigma}$ and $V_{\mathrm{ee}}^{\sigma \tau}$ ($\sigma \neq \tau$) 
for the molecules addressed in this work. The exchange ($V_{\mathrm{X}}^{\sigma \sigma}$)
together with the spin-dependent correlation terms $V_{\mathrm{corr}}^{\sigma \sigma}$ and 
$V_{\mathrm{corr}}^{\sigma \tau}$ are also reported.
Atomic units are used throughout.}

%\vspace*{-1.0cm}

\begin{center}
\hspace*{-1.0cm} \begin{tabular}{l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l|r@{.}l}
\hline
 & \multicolumn{6}{|c}{HF} & \multicolumn{12}{|c}{HF/CC} \\
\hline
System & \multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{total}}$} & 
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\sigma \sigma}$} &
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\sigma \tau}$} & 
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\mathrm{total}}$} & 
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\sigma \sigma}$} &
\multicolumn{2}{c|}{$V_{\mathrm{ee}}^{\sigma \tau}$} &
\multicolumn{2}{c|}{$V_{\mathrm{X}}^{\sigma \sigma}$} &
\multicolumn{2}{c|}{$V_{\mathrm{corr}}^{\sigma \sigma}$} &
\multicolumn{2}{c}{$V_{\mathrm{corr}}^{\sigma \tau}$} \\
\hline
%\ce{CN-} & 54&932008 &   21&532656 &   33&399352 &   54&692365 & 21&513756 &   33&178605  \\
%ce{HCCH} & 49&923145 &   19&478676 &   30&444469 &   49&747864 & 19&489659 &   30&258209 \\
%ce{LiF} & 53&310645 &   20&659249 &   32&651397 &   52&891884 & 20&539863 &   32&352018 \\
%ce{NO+} &  0&000000 &    0&000000 &    0&000000 &   68&539613 & 27&173010 &   41&366591 \\
\ce{BeH2} &  7&915717 &    2&234550 &    5&681168 &    7&838443 &    2&236701 &    5&601742 & $-$3&446740 & $-$0&002012 & $-$0&083711 \\
\ce{BH} &  9&915993 &    2&891689 &    7&024304 &    9&839581 &    2&900865 &    6&938718 & $-$4&134972 & $-$0&006502 & $-$0&103621 \\
\ce{CN-} & 54&932008 &   21&532656 &   33&399352 &   54&692365 &   21&513756 &   33&178605 & $-$11&863202 & $-$0&077487 & $-$0&275840 \\
\ce{HF} & 45&373000 &   17&470029 &   27&902970 &   45&049423 &   17&385098 &   27&664330 & $-$10&432695 & $-$0&042598 & $-$0&196061 \\
\ce{LiF} & 53&310645 &   20&659249 &   32&651397 &   52&891884 &   20&539863 &   32&352018 & $-$11&988489 & $-$0&033823 & $-$0&210157 \\
\ce{NO+} & 68&813436 &   27&197122 &   41&616314 &   68&539613 &   27&173010 &   41&366591 & $-$14&431472 & $-$0&072680 & $-$0&310571 \\
\ce{LiH} &  3&474688 &    0&665519 &    2&809169 &    3&428369 &    0&665924 &    2&762445 & $-$2&143692 & 0&001086 & $-$0&046085 \\
\ce{H2O\bond{...}H2O} & 93&773968 &   37&939638 &   55&834329 &   93&206339 &   37&811657 &   55&394675 & $-$17&890761 & $-$0&092376 & $-$0&400120 \\
\ce{HC#CH} & 49&923145 &   19&478676 &   30&444469 &   49&747864 &   19&489659 &   30&258209 & $-$10&966485 & $-$0&070246 & $-$0&268181 \\
\hline
\ce{CH3.} & 22&385539 &  8&216757 & 14&168783 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}  \\
\ce{CH3CH2.}  & 62&317091 & 25&220541 & 37&096550 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}  \\
\ce{(CH3)2CH.} & 113&489595 & 47&844631 & 65&644964 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}   \\
\ce{(CH3)3C.}  & 176&172545 & 76&224159 & 99&948386 & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---}  & \multicolumn{2}{c|}{---} & \multicolumn{2}{c|}{---} & \multicolumn{2}{c}{---}  \\
\hline
\end{tabular}
\end{center}
\label{tab:VeeTotales}
\end{sidewaystable}%

\thispagestyle{empty}
\thispagestyle{empty}

